Domain Randomization is Sample Efficient for Linear Quadratic Control

We study the sample efficiency of domain randomization and robust control for the benchmark problem of learning the linear quadratic regulator (LQR). Domain randomization, which synthesizes controllers by minimizing average performance over a distribution of model parameters, has achieved empirical success in robotics, but its theoretical properties remain poorly understood. We establish that with an appropriately chosen sampling distribution, domain randomization achieves the optimal asymptotic rate of decay in the excess cost, matching certainty equivalence. We further demonstrate that robust control, while potentially overly conservative, exhibits superior performance in the low-data regime due to its ability to stabilize uncertain systems with coarse parameter estimates. We propose a gradient-based algorithm for domain randomization that performs well in numerical experiments, which enables us to validate the trends predicted by our analysis. These results provide insights into the use of domain randomization in learning-enabled control, and highlight several open questions about its application to broader classes of systems.

==> introduction_unused.tex <==
\section{Introduction_unused}

\sloppy 
Prior work analyzing the sample complexity of learning the linear quadratic regulator has shown that the principle known as certainty equivalence, in which one uses the dataset $\curly{(X_t^n, U_t^n, X_{t+1}^n)}_{t=1, n=1}^{T,N}$ to estimate the dynamics $\hat\theta = \bmat{\hat A & \hat B}$, and then in turn synthesizes a controller as though these parameters were the ground truth as $\hat K = K(\hat \theta)$, 
is efficient \citep{mania2019certainty}.  The notion of efficiency in prior work refers to the fact that the rate of decay suboptimality gap \eqref{eq: suboptimality gap}, asymptotically matches the lower bound, i.e. it decays at the optimal rate the total number of samples $TN$. Follow up analysis by \citet{wagenmaker2021task, lee2024active} has shown the optimal asymptotic dependence on system theoretic constants. 

What prior analysis studying certainty equivalence fails to adequately address is that certainty equivalence may perform very poorly in the low-data regime. In particular, it may be that the certainty equivalent controller does not even stabilize the system when limited data is available. This motivates alternative design methodologies, in which one quantifies the uncertainty in the estimate of $\hat A$ and $\hat B$, and uses this uncertainty quantification to design a robust controller. Common notions of how to do this would be to use robust synthesis, whereby a controller is either synthesized to minimize an objective value in the face of the worst case dynamics realization in a high probability set or minimize the nominal cost while ensuring stability for all systems in a high probability set \citep{gevers2005identification, dean2020sample}. Alternatively, $\calH_\infty$ or mixed $\calH_2/\calH_\infty$ methods can be used to design systems which are robust to feedback uncertainty, as guaranteed by the small gain theorem \citep{zhou1996robust}. 
There are severe limitations to these approaches. 
\begin{enumerate}
    \item It is challenging to derive computationally feasible extensions of either of these approaches to general classes of nonlinear systems. 
    \item The increasingly adopted approaches of performing approximate dynamic programming to perform optimal control via policy approximation (typically with neural networks) are not easily amenable to these conventional approaches for incorporating robustness. 
    \item Robust synthesis can be overly conservative. Indeed, while some existing finite sample bounds exist for robust synthesis \citep{dean2020sample}, the rate of decay is linear the estimation error rather than quadratic. This limitation is not fundamental (as we show in this work.) However, suptoptimal dependence on the system theoretic constants may be fundamental (as we conjecture in this work). 
    \item Analyzing the sample complexity of certainty equivalence with stability constraints is not straightforward in the regime where the constraints are active. 
\end{enumerate}

\section{Excess cost analysis}
Define the \emph{model-task Hessian} of the LQR problem as 
\begin{align*}
    H(\tilde \theta) = \nabla_{\theta}^2 J(K(\theta), \tilde \theta) \vert_{\theta= \tilde \theta}.
\end{align*}
Additionally, let
\begin{align*}
    \Psi(\theta) &= B(\theta)^\top P(\theta) B(\theta) + R \\
    \Sigma_{\tilde K}(\theta) &= \sum_{t=0}^\infty (A(\theta) + B(\theta) \tilde K)^t \Sigma_W\paren{(A(\theta) + B(\theta) \tilde K)^t }^\top
\end{align*}

\begin{theorem}
    \label{thm: CE bound}
    Let $\hat K = \argmin_K C(K \hat \theta)$. Suppose that 
    \[
        \norm{\hat \theta - \theta^\star} \leq \mathsf{poly}(\norm{P(\theta_\star)}^{-1})
    \]
    Then
    \begin{align*}
        C(\hat K, \theta^\star) - C(K^\star, \theta^\star) \leq (\hat\theta - \theta^\star)^\top H(\theta^\star) (\hat \theta - \theta^\star) + L_{LQR} \norm{\hat \theta - \theta^\star}^3, 
    \end{align*}
    where 
    \begin{align*}
        L_{\mathsf{cost}} \leq \mathsf{poly}(\norm{P(\theta_\star)}, \norm{B}).
    \end{align*}
\end{theorem}
\begin{proof}
    {\color{red} Tesshu will fill in}
\end{proof}

\begin{lemma}
    Let $\hat K = \argmin_K \sup_{\theta\in\calB} C(K,  \theta) - C(K(\theta), \theta)$, where $\calB = \curly{\theta: (\theta - \hat\theta)^\top G (\theta - \hat \theta) \leq 1}$.  Suppose that $\theta_\star \in \calB$. Then
    \begin{align*}
        C(\hat K, \theta^\star) - C(K^\star, \theta^\star) \leq \inf_{\tilde \theta \in \calB} \paren{ 2 \norm{D \VEC K(\theta)\vert_{\theta= \theta_1}^\top (\Psi(\theta_1) \otimes \Sigma_{K(\tilde \theta)}(\theta_1)) D \VEC K(\theta)\vert_{\theta= \theta_1} G} + 2 L_{\mathsf{h.o.t.}}(\tilde \theta) \norm{G}^{3/2}}
    \end{align*}
\end{lemma}
\begin{proof}
    \begin{align*}
        C(\hat K, \theta^\star) - C(K^\star, \theta^\star)  &\leq \sup_{\theta: (\theta - \hat \theta)^\top G (\theta - \hat\theta) \leq 1} C(\hat K, \theta) - C(K(\theta), \theta) \\
        & = \inf_{\tilde K} \sup_{\theta: (\theta - \hat \theta)^\top G (\theta - \hat\theta) \leq 1} C(\tilde K, \theta) - C(K(\theta), \theta) \\
        &= \inf_{\tilde K} \sup_{\theta: (\theta - \hat \theta)^\top G (\theta - \hat\theta) \leq 1} \trace\paren{(\tilde K - K(\theta))^\top \Psi(\theta) \paren{\tilde K - K(\theta)} \Sigma_{\tilde K}(\theta)} \\
        &\leq \inf_{\tilde \theta \in \calB} \sup_{\theta_1, \theta_2\in\calB} \trace\paren{(K(\theta_2) - K(\theta_1))^\top \Psi(\theta_1) \paren{K(\theta_2) - K(\theta_1)} \Sigma_{K(\tilde \theta)}(\theta_1)},
    \end{align*}
    where the inequality follows from the fact that for $S_1 \subseteq S_2$, $\inf_{x \in S_2} f(x,x) \leq \inf_{x \in S_1} f(x,x) \leq \inf_{x \in S_1} \sup_{y\in S_1} f(x,y)$. Taylor expanding $K$ with respect to $\theta$ results in the upper bound of 
    \begin{align*}
        \inf_{\tilde \theta \in \calB} \paren{\sup_{\theta_1, \theta_2\in\calB} (\theta_2 - \theta_1) D \VEC K(\theta)\vert_{\theta= \theta_1}^\top (\Psi(\theta_1) \otimes \Sigma_{K(\tilde \theta)}(\theta_1)) D \VEC K(\theta)\vert_{\theta= \theta_1} (\theta_2 - \theta_1) + \sup_{\theta_1, \theta_2\in\calB}  L_{\mathsf{h.o.t.}} (\tilde \theta) \norm{\theta_2 - \theta_1}^3},
    \end{align*}
    where $L_{\mathsf{h.o.t.}} = ?$ \textcolor{red}{Work out the higher order terms from the derivative}. Taking the supremum over $\theta_1$ and $\theta_2$ thus leads to the upper bound
    \begin{align*}
         \inf_{\tilde \theta \in \calB} \paren{ 2 \norm{D \VEC K(\theta)\vert_{\theta= \theta_1}^\top (\Psi(\theta_1) \otimes \Sigma_{K(\tilde \theta)}(\theta_1)) D \VEC K(\theta)\vert_{\theta= \theta_1} G} + 2 L_{\mathsf{h.o.t.}}(\tilde \theta) \norm{G}^{3/2}}
    \end{align*}
    
    % {\color{red} Use the fact that both $\tilde K$ and $K$ stabilize the system to bound
    % \begin{align*}
    %     \norm{\Sigma_{\tilde K}(\theta)- \Sigma_{K(\theta)}(\theta)} \leq  \norm{\dlyap(A+BK(\theta))} \\ \paren{2 \norm{A+B K(\theta)} \norm{\Sigma_{\tilde K}} \norm{B} \norm{\tilde K - K(\theta)} + \norm{\Sigma_{\tilde K}} \norm{B}^2 \norm{\tilde K - K(\theta)}^2}
    % \end{align*} 
    % $\norm{\Sigma_{\tilde K}}$ can then be bounded by $\norm{\Sigma_{K(\theta)}} + \norm{\Sigma_{\tilde K} - \Sigma_{K(\theta)}}$. Under a closeness condition on $\tilde K$, this in turn can imply a bound on $\norm{\Sigma_{\tilde K} - \Sigma_{K(\theta)}}$ in terms of $\tilde K - K(\theta)$.
    % }
\end{proof}

If $\hat \theta$ is identified from data via least squares, then for any $\delta$, we can construct a matrix $G$ such that $\theta_\star \in \calB$ with probability at least $1-\delta$ as $G = $ empirical covariance divided by confidence scaling. This leads to the following result:
\begin{theorem}
Suppose data is collected ... Then .
\end{theorem}
Notably, the above upper bound may be finite even in situations where the certainty equivalent controller is not stabilizing. In particular, consider the system $A = 0.99$, $B = 1$ with $Q= 1e-3$ and $R=1$ - {\color{red} work out an amount of data where CE is not stabilizing with high probability, whereas DR is.} Nonetheless, a rate of decay of $\frac{1}{N}$ is achieved asymptotically, matching the analysis of \citet{mania2019certainty} for certainty equivalence, and improving upon the $1/\sqrt{N}$ rate of \citet{dean2020sample} for robust synthesis. However, the bound does not achieve the optimal asymptotic dependence on system theoretic parameters. In particular, \Cref{thm: CE bound} shows that certainty equivalence achieves the bound $\trace\paren{H(\theta^\star) \mathsf{FI}(\theta^\star)^{-1}}$.

Motivated by the above limitations, we study an approach to controller synthesis rooted in domain randomization. In particular, using the dataset $\curly{(X_t^n, U_t^n, X_{t+1}^n)}_{t=1, n=1}^{T,N}$, we construct a parameter distribution $\calD$, and select the controller as
\begin{align}
    \label{eq: domain randomization}
    \hat K = \argmin_{K} \E_{\boldsymbol \theta \sim \calD} \brac{C(K, \boldsymbol \theta)}. 
\end{align}

Our main result is a bound on the suboptimality gap incurred by rolling out a controller synthesized with domain randomization. This result is stated informally below.

\begin{theorem}[(Main Result)]
    \label{thm: informal main result}
    Let $\hat K$ be generated according to \eqref{eq: domain randomization}. Then the suboptimality gap satisfies
    \begin{align*}
        &C(\hat K, \theta^\star) - C(K(\theta^\star), \theta^\star) \leq  \trace(\var(\theta) \cdot H(\theta^\star)) + \left(\E[\theta] - \theta^\star\right)^\top H(\theta^\star) \left(\E[\theta] - \theta^\star\right) + \text{h.o.t.},
    \end{align*}
    where $H(\theta^\star)$ is the \textit{model-task Hessian}. The above bound holds whenever $\hat K$ robustly stabilizes the true system parameters $\theta^\star = \bmat{A^\star & B^\star}$.
\end{theorem}

\begin{proof}
    Our result proceeds by the observations that 

\end{proof}

We contrast this result with the analogous bound for certainty equivalence: as long as $K(\hat \theta)$ robustly stabilizes $\theta^\star$,
\begin{equation}
\label{eq: certainty equivalence suboptimality gap}
\begin{aligned}
    &C(K(\hat \theta), \theta^\star) - C(K(\theta^\star), \theta^\star) \leq \trace\left((\hat \theta - \theta^\star)^\top H (\hat \theta - \theta^\star)\right) + \text{h.o.t.}.
\end{aligned}
\end{equation}

At first glance, the upper bound for domain randomization (\Cref{thm: informal main result}) appears to be worse than the one for certainty equivalence. The key reason this is not the case lies in the stability assumptions. Domain randomization ensures that $\hat K$ robustly stabilizes all parameters $\theta = \bmat{A & B}$ with non-zero support in the distribution $\calD$, whereas certainty equivalence requires the parameters $\hat A$ and $\hat B$ to be very close to the true values $A^\star$ and $B^\star$. This discrepancy shows up in the required data collection to achieve the respective performance bounds.

We now briefly return to the robust synthesis problem. 

\begin{theorem}
    Suppose that $\hat K$ is generated by
    \begin{align*}
        \hat K = \argmin_K \sup_{\theta \in \calB} C(K, \theta).
    \end{align*}
    Then the suboptimality gap is bounded by
    \begin{align*}
        &C(\hat K, \theta^\star) - C(K(\theta^\star), \theta^\star) \\
        &\leq \sup_{\theta \in \calB} \VEC(\theta - \theta^\star)^\top H \VEC(\theta - \theta^\star) + \text{h.o.t.}.
    \end{align*}
\end{theorem}

Crucially, even if we shrink the diameter of the uncertainty set $\calB$ based on parameter estimation uncertainty, the suboptimality gap for robust synthesis includes a term scaling with $\norm{H \mathsf{FI}^{-1}}$, whereas domain randomization and certainty equivalence instead involve a term scaling as $\trace(H \mathsf{FI}^{-1})$.

\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{figures/Excess_cost.png}
    \caption{Excess cost comparison between Certainty Equivalence (CE) and Domain Randomization (DR).}
    \label{fig:excess cost}
\end{figure}


% Our main result is a bound on the suboptimality gap incurred by rolling out a controller synthesized with domain randomization. This result is stated informally below. 
% \begin{theorem}[(informal, main result)]
%     \label{thm: informal main result}
%     Let $\hat K$ be generated according to \eqref{eq: domain randomization}. Then the subpotimality gap satisifes
%     \begin{align*}
%         &C(\hat K, \bmat{A_\star & B_\star}) - C(K(\bmat{A_\star & B_\star}), \bmat{A_\star & B_\star})  \\
%         &\leq  \trace(\var(\bmat{\bfA & \bfB})\cdot H^\star) + \left(\mathbf{E}\bmat{\bfA & \bfB} - \bmat{A_\star & B_\star}\right)^T H^\star \left(\mathbf{E}\bmat{\bfA & \bfB} - \bmat{A_\star & B_\star}\right) + h.o.t
%     \end{align*}
%     where $H^\star$ is the \textit{model-task hessian}. The above bound holds whenever $\hat K$ robustly stabilizes $\bmat{A_\star & B_\star}$. 
% \end{theorem}

% We contrast this result with the analog for certainty equivalence: As long as $K(\bmat{\hat A & \hat B})$ robustly stabilizes $\bmat{A_\star & B_\star}$,
% \begin{equation}
% \label{eq: certainty equivalence subtoptimality gap}
% \begin{aligned}
%     &C(K(\bmat{\hat A & \hat B}), \bmat{A_\star & B_\star}) - C(K(\bmat{A_\star & B_\star}), \bmat{A_\star & B_\star}) \\
%     &\leq \trace(\paren{\bmat{\hat A & \hat B} - \bmat{A_\star & B_\star}} H \paren{\bmat{\hat A & \hat B} - \bmat{A_\star & B_\star}}) + h.o.t.
% \end{aligned}
% \end{equation}

% It appears that the upper bound for domain randomization (\Cref{thm: informal main result}) is strictly worse than the one for certainty equivalence. The key to why this is not so is in the stability assumptions. Domain randomization effortlessly ensures that $\hat K$ is stabilizing all parameters $\bmat{A & B}$ with nonzero support in the probability distribution $\calD$, whereas certainty equivalence needs the parameters $\hat A$ and $\hat B$ very close to ground truth. This discrepancy shows up in the burn-in times (amount of sampled data required to achieve the above bounds). 

% It is worth returning briefly to the problem of robust synthesis. 
% \begin{theorem}
%     Suppose that $\hat K$ is given by
%     \begin{align*}
%         \argmin_K \sup_{\bmat{A & B} \in \calB} C(K, \bmat{A & B}).
%     \end{align*}
%     Then the suboptimality gap is bounded by
%     \begin{align*}
%         &C(\hat K, \bmat{A_\star & B_\star}) - C(K(\bmat{A_\star & B_\star}), \bmat{A_\star & B_\star}) \\ 
%         &\leq \sup_{\bmat{A & B} \in \calB} \VEC \bmat{A - A_\star & B - B_\star}^\top H \VEC \bmat{A - A_\star & B - B_\star} + h.o.t.
%     \end{align*}
% \end{theorem}
% Critically, even if we shrink the diameter of the ball $\calB$ in the above robust synthesis according to the uncertainty in the parameter estimates, the suboptimality gap above picks up a quantity scaling as $\norm{H \mathsf{FI}^{-1}}$, whereas domain randomization and certianty equivalence instead pick up a term scaling like $\trace\paren{H \mathsf{FI}^{-1}}$. 

% \begin{figure}
%     \centering
%     \includegraphics[width=1.0\linewidth]{figures/Excess_cost.png}
%     \caption{Excess Cost between CE vs. DR}
%     \label{fig:excess cost}
% \end{figure}

\Bruce{TODO 
- Add preliminary plot for proof of concept experiments
- verify proof sketch of the main result
}

==> several_interesting_notes.tex <==
\section{Several interesting notes}

% \subsection{Solving the domain randomized LQR problem}

% Unfortunately, I think this subsection is a rabbit whole that can be chalked up to a waste of time. (Not quite, this is a different formulation of domain randomization that could still be useful, where $\theta$ at any time is sampled randomly.) But useless for what we want to prove. 

% \begin{lemma}[Stochastic Dynamic Programming for Domain Randomized LQR]
%     Consider the finite-horizon linear quadratic regulator problem with uncertain system matrices. The state evolves as
%     \[
%     X_{t+1} = A X_t + B U_t + W_t,
%     \]
%     where the system matrices $\theta = \bmat{A & B}$ are sampled from a distribution $\mathcal{D}(\theta)$, and $W_t \sim \mathcal{N}(0, \Sigma_w)$ is Gaussian noise. The finite-horizon quadratic cost is given by
%     \[
%     \mathbb{E}_{\theta \sim \mathcal{D}}\left[\sum_{t=0}^{T-1} \left( X_t^\top Q X_t + U_t^\top R U_t \right) + X_T^\top Q_T X_T \right],
%     \]
%     where $Q \succeq 0$, $R \succ 0$, and $Q_T \succeq 0$ are known cost matrices. \Bruce{I'm not even sure this part is correct. Actually, I really don't think it is. $\theta$ is not drawn iid at every instance, and therefore, is not independent of the observed states. Principle of optimality does not hold. Verify this intuition.}

%     The optimal control law $U_t = -K_t X_t$ that minimizes the expected cost is computed via the following backward recursion:
%     \begin{align*}
%         P_T &= Q_T, \\
%         P_t &= Q + \mathbb{E}_{\theta \sim \mathcal{D}}\left[A^\top P_{t+1} A\right] - \mathbb{E}_{\theta \sim \mathcal{D}}\left[A^\top P_{t+1} B\right]
%         \left(\mathbb{E}_{\theta \sim \mathcal{D}}\left[B^\top P_{t+1} B\right] + R\right)^{-1}
%         \mathbb{E}_{\theta \sim \mathcal{D}}\left[B^\top P_{t+1} A\right],
%     \end{align*}
%     where $P_t$ is the cost-to-go matrix at time $t$ and the control gain is given by
%     \[
%     K_t = \left(\mathbb{E}_{\theta \sim \mathcal{D}}[B^\top P_{t+1} B] + R \right)^{-1} \mathbb{E}_{\theta \sim \mathcal{D}}[B^\top P_{t+1} A].
%     \]
% \end{lemma}

% \begin{proof}
%     We solve the problem using stochastic dynamic programming, assuming that the cost-to-go function is quadratic at each time step, as in the classical LQR problem. Let $J_t(X_t)$ denote the cost-to-go function at time $t$. We define the Bellman recursion for the finite-horizon problem as follows:
%     \[
%     J_T(X_T) = X_T^\top Q_T X_T,
%     \]
%     and for $t = T-1, \dots, 0$, the recursion is given by:
%     \[
%     J_t(X_t) = \min_{U_t} \mathbb{E}_{\theta \sim \mathcal{D}}\left[X_t^\top Q X_t + U_t^\top R U_t + \mathbb{E}[J_{t+1}(X_{t+1}) | X_t, U_t]\right].
%     \]

%     The state evolves as $X_{t+1} = A X_t + B U_t + W_t$, where $A$ and $B$ are drawn from the distribution $\mathcal{D}(\theta)$. Substituting this into the cost-to-go function:
%     \[
%     J_t(X_t) = \min_{U_t} \mathbb{E}_{\theta \sim \mathcal{D}}\left[X_t^\top Q X_t + U_t^\top R U_t + \mathbb{E}\left[J_{t+1}(A X_t + B U_t + W_t)\right]\right].
%     \]

%     Assume that $J_{t+1}(X_{t+1}) = X_{t+1}^\top P_{t+1} X_{t+1}$ is quadratic in $X_{t+1}$. Then,
%     \[
%     \mathbb{E}[J_{t+1}(X_{t+1})] = \mathbb{E}_{\theta \sim \mathcal{D}} \left[ (A X_t + B U_t)^\top P_{t+1} (A X_t + B U_t) + \text{tr}(P_{t+1} \Sigma_w) \right].
%     \]
%     Expanding this expression yields:
%     \begin{align*}
%     \mathbb{E}[J_{t+1}(X_{t+1})] &= X_t^\top \mathbb{E}_{\theta \sim \mathcal{D}}\left[A^\top P_{t+1} A\right] X_t + 2 X_t^\top \mathbb{E}_{\theta \sim \mathcal{D}}\left[A^\top P_{t+1} B\right] U_t \\&+ U_t^\top \mathbb{E}_{\theta \sim \mathcal{D}}\left[B^\top P_{t+1} B\right] U_t + \text{tr}(P_{t+1} \Sigma_w).
%     \end{align*}

%     Substituting this into the Bellman recursion for $J_t(X_t)$, we obtain:
%     \begin{align*}
%     J_t(X_t) &= \min_{U_t} \Bigg( X_t^\top Q X_t + U_t^\top R U_t + X_t^\top \mathbb{E}_{\theta \sim \mathcal{D}}[A^\top P_{t+1} A] X_t \\&+ 2 X_t^\top \mathbb{E}_{\theta \sim \mathcal{D}}[A^\top P_{t+1} B] U_t + U_t^\top \mathbb{E}_{\theta \sim \mathcal{D}}[B^\top P_{t+1} B] U_t + \text{tr}(P_{t+1} \Sigma_w) \Bigg).
%     \end{align*}

%     This is a quadratic expression in $X_t$ and $U_t$. The optimal control law $U_t = -K_t X_t$ can be computed by solving for $K_t$:
%     \[
%     K_t = \left(\mathbb{E}_{\theta \sim \mathcal{D}}[B^\top P_{t+1} B] + R \right)^{-1} \mathbb{E}_{\theta \sim \mathcal{D}}[B^\top P_{t+1} A].
%     \]

%     Substituting the optimal $U_t = -K_t X_t$ back into the Bellman equation gives the Riccati-like recursion:
%     \[
%     P_t = Q + \mathbb{E}_{\theta \sim \mathcal{D}}[A^\top P_{t+1} A] - \mathbb{E}_{\theta \sim \mathcal{D}}[A^\top P_{t+1} B] \left(\mathbb{E}_{\theta \sim \mathcal{D}}[B^\top P_{t+1} B] + R \right)^{-1} \mathbb{E}_{\theta \sim \mathcal{D}}[B^\top P_{t+1} A].
%     \]
% \end{proof}

% \begin{lemma}[Infinite Horizon Stochastic LQR]
%     Consider the infinite-horizon linear quadratic regulator problem with uncertain system matrices. The state evolves as
%     \[
%     X_{t+1} = A X_t + B U_t + W_t,
%     \]
%     where the system matrices $\theta = \bmat{A & B}$ are sampled from a distribution $\mathcal{D}(\theta)$, and $W_t \sim \mathcal{N}(0, \Sigma_w)$ is Gaussian noise. The infinite-horizon quadratic cost is defined as the limiting average cost:
%     \[
%     \limsup_{T \to \infty} \frac{1}{T} \mathbb{E}_{\theta \sim \mathcal{D}} \left[ \sum_{t=0}^{T-1} \left( X_t^\top Q X_t + U_t^\top R U_t \right) \right],
%     \]
%     where $Q \succeq 0$ and $R \succ 0$ are known cost matrices.

%     The optimal time-invariant control law $U_t = -K_\infty X_t$ is computed by solving the following \textbf{stochastic Riccati equation}:
%     \[
%     P_\infty = Q + \mathbb{E}_{\theta \sim \mathcal{D}}[A^\top P_\infty A] - \mathbb{E}_{\theta \sim \mathcal{D}}[A^\top P_\infty B] \left( \mathbb{E}_{\theta \sim \mathcal{D}}[B^\top P_\infty B] + R \right)^{-1} \mathbb{E}_{\theta \sim \mathcal{D}}[B^\top P_\infty A],
%     \]
%     where $P_\infty$ is the steady-state solution to the stochastic Riccati equation. The optimal feedback gain is given by
%     \[
%     K_\infty = \left(\mathbb{E}_{\theta \sim \mathcal{D}}[B^\top P_\infty B] + R \right)^{-1} \mathbb{E}_{\theta \sim \mathcal{D}}[B^\top P_\infty A].
%     \]
% \end{lemma}

% \begin{proof}
%     \Bruce{This proof is wrong. Conjecture: it requires an assumption that the support of $\calD$ is jointly stabilizable. }
%     The proof proceeds by solving the Bellman equation for the infinite-horizon problem. Instead of directly summing the cost over an infinite horizon, we focus on the limiting average cost:
%     \[
%     \limsup_{T \to \infty} \frac{1}{T} \mathbb{E}\left[ \sum_{t=0}^{T-1} \left( X_t^\top Q X_t + U_t^\top R U_t \right) \right].
%     \]
%     As in the classical LQR case, we assume that the cost-to-go function is quadratic in $X_t$ for large $t$, i.e., $J(X_t) = X_t^\top P_\infty X_t$, which leads to a time-invariant solution. However, since $A$ and $B$ are random variables drawn from $\mathcal{D}(\theta)$, the Riccati recursion involves expectations over these parameters. Taking the limit of the Riccati recursion from the finite-horizon case as $t \to \infty$ yields the steady-state solution $P_\infty$. The control law $U_t = -K_\infty X_t$ follows by minimizing the quadratic cost at each time step.
% \end{proof}

% Interestingly, the above lemma may provide us with a deterministic algorithm to compute the domain randomized controller. In particular, as long as the iterations converge, the stochastic Riccati equation can be solved via recursion by computing the first and second moments of the parameter distribution. There is some subtlety involved though, which I have not entirely wrapped my head around. In particular, observe the following points:
% \begin{itemize}
%     \item The domain randomized controller only depends on the first and second moments of the parameter distribution. 
%     \item One can construct two parameter distribution with the same first and second moments. However, one may construct them such that the systems in the support of one parameter distribution are jointly stabilizable, however the systems in the support of the other are not. 
%     \item If the systems in the support of the parameter distribution are not jointly stabilizable, then the expected LQR cost is infintie. 
%     \item This means that even if the stochastic Riccati equation converges, it does not necessarily hold that the resultant controller stabilizes the support of $\calD$. In particular, it is not necessarily true that
%     \begin{align*}
%         \trace(P_{\infty} \Sigma_w) = \mathbb{E}_{\theta\sim \calD}\brac{C(K, \theta)}. 
%     \end{align*}
% \end{itemize}
%  I have not formalized an explanation for the above discussion; however, I conjecture that the subtlety partially arises in moving to the infinite horizon setting as objectives become unbounded. In particular, the issue likely arises due to the interchange in the order of expectation, which is permitted only under boundedness of the integrands. This boundedness should come, however, if there is an assumption that the support of $\calD$ is jointly stabilizable. This should be formalized, as it would give us a very effective algorithm in the setting where the support of the distribution is stabilizable. 

 \subsection{Misspecification}

 This paper has focused on a situation where domain randomization is used to mitigate the uncertainty in the model due to variance in fitting the model. In particular, assuming the dynamics \eqref{eq: linear system} imposes a realizability assumption. Thereby, an appropriatley constructed distribution $\calD$ contains $\theta^\star$ in the support with high probability. 

 However, one of the explanations posited for the empirical success of domain randomization in many robotics examples \citep{?} is that domain randomization fares well in the presence of misspecification. In particular, this consists of settings where the true system is not represented by the set of dynamics described by the distribution of parameters $\calD$. In this paper, we do not delve into this topic in depth. However, we do believe it is a valuable direction for future investigation. 

  Consider a scalar linear dynamical system:
     \begin{align*}
        X_{t+1} = a^\star X_t + b^\star U_t + W_t \quad \forall t\geq 0,
     \end{align*}
    where $a^\star = 1.05$ and $b^\star = 1$.  
    
    Suppose that the actuation matrix was assumed to be known; however, this assumption was incorrect. In particular, suppose that the engineer's esimate for the actuation is $\hat b = 1.0$. Suppose that $a^\star$ was assumed to be unknown, and through a system identification procedure, the engineer determined an estimate $\hat a = 1.1$. 
    
    If the engineer attempts to minimize an LQR objective with $Q=1$ and $R=1000$, they will synthesize a controller
    \[
        \hat k = K(\bmat{\hat a & \hat b}) = -.195.  
    \]
    This controller does not stabilize the true system, as the closed-loop state matrix is $a^\star + \hat k b^\star = 1.0024$. 
    
    However, if the engineer applies domain randomization over the $a$ parameter with the distribution $\calD = U[0.9, 1.3]$, and synthesizes a controller as 
    \[
        \hat k = \argmin_{k} \mathbb{E}_{a\sim U[1.0, 1.2]} \brac{C(k, \bmat{a & \hat b})} = -0.206,
    \]
    the closed-loop state matrix is $a^\star + b^\star \hat k = 0.997$, which is stable.  
    
 
 % To provide a starting place for such investigations, we provide a simple proof of concept example where domain randomization yields a benefit over certainty equivalence in a situation consisting of misspecification. 



